Imaginative Walks: Generative Random Walk Deviation Loss for Improved Unseen Learning Representation

We propose a novel loss for generative models, dubbed as GRaWD (Generative Random Walk Deviation), to improve learning representations of unexplored visual spaces. Quality learning representation of unseen classes (or styles) is critical to facilitate novel image generation and better generative understanding of unseen visual classes, i.e., zero-shot learning (ZSL). By generating representations of unseen classes based on their semantic descriptions, e.g., attributes or text, generative ZSL attempts to differentiate unseen from seen categories. The proposed GRaWD loss is defined by constructing a dynamic graph that includes the seen class/style centers and generated samples in the current minibatch. Our loss initiates a random walk probability from each center through visual generations produced from hallucinated unseen classes. As a deviation signal, we encourage the random walk to eventually land after t steps in a feature representation that is difficult to classify as any of the seen classes. We demonstrate that the proposed loss can improve unseen class representation quality inductively on text-based ZSL benchmarks on CUB and NABirds datasets and attribute-based ZSL benchmarks on AWA2, SUN, and aPY datasets. In addition, we investigate the ability of the proposed loss to generate meaningful novel visual art on the WikiArt dataset. The results of experiments and human evaluations demonstrate that the proposed GRaWD loss can improve StyleGAN1 and StyleGAN2 generation quality and create novel art that is significantly more preferable. Our code is made publicly available at https://github.com/Vision-CAIR/GRaWD.

==> approach_old.tex <==

%\textbf{Generative Random Walk  Deviation loss}. 

% Our goal is to have points of the same class form a compact cluster in latent space, well separated from other classes. 

We start by defining our loss for \emph{Generative Zero-Shot Learning.} We will show in our experiments how it can be integrated with state-of-the-art GAN models to encourage novel generations. 
Let's denote the set of seen and unseen class labels as $\mathcal{S}$ and $\mathcal{U}$, where $\mathcal{S} \cap \mathcal{U} = \emptyset$. We denote the semantic representations of unseen classes and seen classes as $s_u=\psi(T_u) \in \mathcal{T}$ and $s_i=\psi(T_i) \in \mathcal{T}$ respectively, where $\mathcal{T}$ is the semantic space and $\psi(\cdot)$ is the semantic description function that extract features from text article or attribute description of class $k$. 
Let's denote the seen data as $D^s = \{(x_i^s, y_i^s, s_i) \}$,  where $x_i^s \in \mathcal{X}$ denotes the visual features of the $i^{th}$ image, $y_i^s \in \mathcal{S}$ is the corresponding seen category label. 
For unseen classes, we are given only their semantic representations, one per class, $s_u$. We define  $K^u$ as the number of unseen classes. In Generalized ZSL (GZSL), we aim to predict the label  $y \in \mathcal{U} \cup \mathcal{S}$ at test time given  $x$ that may belong to seen or unseen classes. 


We denote the generator as $G$:  $\mathbb{R}^Z \times \mathbb{R}^T \xrightarrow{\theta_G} \mathbb{R}^X$ and  the discriminator as $D$ : $\mathbb{R}^X \xrightarrow{\theta_D} \{0,1\} \times\{1 \cdots  K^s\} $, where  $\theta_G$ and $\theta_D$ are parameters of the generator and the discriminator as  respectively,  $\{ 1 \cdots K^s\}$ is the set of seen class labels; see Fig.~\ref{fig1approach}. For the Generator $G$ and as in ~\cite{xian2018feature,Elhoseiny_2018_CVPR,elhoseiny2019creativity,felix2018multi}, the semantic representation is concatenated with a random vector $z \in \mathbb{R}^Z$ sampled from a Gaussian distribution $p_z=\mathcal{N} (0,1)$. 
The discriminator $D$ is trained with two objectives: (1)   predict real for images from the training images and fake for generated ones. (2)  identify the category of the input image.  The discriminator then has two heads. The first head is for binary real/fake classification; $\{0,1\}$ classifier. The second head is a $K^s$-way classifier over the seen classes. 
We denote the  real/fake probability produced by $D$ for an input image as $D^r(\cdot)$, and the classification score of a seen class $k \in \mathcal{S}$  given the image as $D^{s,k}(\cdot)$. Hence, $ G (z, s_k)$ are the  generated features from the semantic description $s_k$ of class $k$. 





\vspace{-1mm}
\subsection{Generative Random Walk Deviation  Loss}
% \kai{we're trying to improve the performance of tf-vaegan on attribute-based datasets.}

 We generate $N_u$ representations in the current current minibatch that we aim to deviate from the seen classes. We denote these hallucinated feature representations as $X_u = \{x^u_1 \cdots x^u_{N_u}\} $, which are    is sampled by $\phi(G (z, s_u))$ where $z \sim
 p_z=\mathcal{N}(0,I)$,  $s_u  \sim p_u$ is a semantic description of a hallucinated unseen class;  $p_u$ is defined in the next section. $\phi(\cdot)$ is a feature extraction function that we used as the features from the last layer of the Discriminator $D$ followed by scaled L2 normalization $L2(\mathbf{v},\beta) = \beta \frac{ \mathbf{v}}{\| \mathbf{v} \|}$; the scaled factor  is mainly to amplifying the norm of the vectors to avoid the vanishing gradient problem inspired from~\cite{bell2016inside}. We used $\beta=3$ in our experiments guided by~\cite{bell2016inside,zhang2019large}. 
% We represent seen classes in the same feature apace as $X_u$, as $C = \{ \mathbf{c}_1 \cdots \mathbf{c}_{K^s}\}$, where $\mathbf{c}_i \in \mathbb{R}^{D}$ represents center of class $i$ that we defined as $\mathbf{c}=\phi(G(z = \mathbf{0}, s_i))$,  where $s_i$ is the attribute or text description of seen class $i$. 
We represent seen classes as $C = \{ \mathbf{c}_1 \cdots \mathbf{c}_{K^s}\}$, where $\mathbf{c}_i$ represents center of class $i$ that we defined as
\begin{equation}
    \mathbf{c}_i=\phi(G(z = \mathbf{0}, s_i))
\end{equation}
 where $s_i$ is the attribute or text description of seen class $i$. 
Let $B \in \mathbb{R}^{N_u\times K^s}$ be the similarity matrix between each of the features of the generations ($x^u \in X_u$ ) and the cluster centers ($c \in C$ ). Similarly, let $A \in \mathbb{R}^{N_u \times N_u }$ compute the similarity matrix between the generated points. In particular,  we use the negative Euclidean distances between the embeddings as a similarity measure as follows:  
\begin{equation}
    B_{ij} = -\|x_i - \mathbf{c}_j \|^2, \,\,\, A_{i,j} = -\|x^u_i - x^u_j\|^2
\end{equation}
where $x^u_i$ and $x^u_j$ are $i^{th}$ and  $j^{th}$ features in the set $X_u$; see Fig.~\ref{fig1approach}. To avoid self-cycle, The diagonal entries $A_{i,i}$ are set to a small number $\epsilon$.  
%Based on A and B, we defined three transition probability matrices $P^{\mathbf{C} \rightarrow X_u} = \textup{softmax}(B^\mathbb{T})$. The softmax operator is applied over each row of the input $B^T$ matrix and hence  $P^{\mathbf{C} \rightarrow X_u}$  represents the transition from each seen class over the $N_u$ generated points. We similarly define $P^{ X_u \rightarrow \mathbf{C }} =  softmax (B)$ as the transition probability from each point over the $K_s$ seen classes. The last transition probability matrix is  $P^{ X_u \rightarrow X_u} = softmax(A)$ from each generated point to over other generated points while avoiding self-loops as we mentioned earlier.  We define our generative random walker probability matrix as: 
Hence, 
we defined three transition probability matrices:
\begin{equation}
\small
   P^{\mathbf{C} \rightarrow X_u} = {\sigma}(B^\mathbb{T}),\,\,\,  P^{ X_u \rightarrow \mathbf{C }} =  \sigma (B),\,\,\, P^{ X_u \rightarrow X_u} = \sigma(A) 
\end{equation}
where $\sigma$ is the softmax operator is applied over each row of the input matrix,  
\noindent  $P^{\mathbf{C} \rightarrow X_u}$ and $P^{ X_u \rightarrow \mathbf{C }}$ are the transition probability matrices from each seen class over the $N_u$ generated points and vice-versa respectively.  $P^{ X_u \rightarrow X_u}$ is the transition probability matrix from each generated point over other generated points. 
%\noindent  $P^{ X_u \rightarrow \mathbf{C }} =  softmax (B)$:  from each generated point over the $K_s$ seen classes. 
%\noindent  $P^{ X_u \rightarrow X_u} = softmax(A)$ from each generated point to over other generated points.% while avoiding self-loops as we mentioned earlier. 
We hence define our generative random walker probability matrix as: 
\begin{equation}\label{eq:rw}
\small
    P^{\mathbf{C } \rightarrow \mathbf{C }} (t, X_u) = {\sigma}(B^\mathbb{T}) \cdot ( \sigma(A))^t \cdot \sigma (B)  
\end{equation}
where  $P^{\mathbf{C } \rightarrow \mathbf{C }}_{i,j} (t, X_u)$ denotes the probability of ending a random walk of a length $t$ at a seen class $j$ {given} that we have started at seen class $i$;   $t$ denotes the number of steps taken between the generated points, before stepping back to land on a seen class. 

 \textbf{Loss: } We construct a random walk loss that encourages unseen visual spaces to deviate from seen classes. 
Hence we defined our loss by encouraging each row in   $P^{\mathbf{C } \rightarrow \mathbf{C }} (t)$ to be hard to classify to seen classes as follows 
\begin{equation}
\small
\begin{aligned}
  {L}_{GRW}(X_u) =& - \sum_{t=0}^{T} {\gamma^{t} \cdot  \sum_{i=1}^{K^s} \sum_{j=1}^{K^s} {U}_c (j) log( {P_{i,j}^{\mathbf{C } \rightarrow \mathbf{C }}}(t,X_u) )}\\
  &-  \sum_{j=1}^{N_u} {U}_x(j)    log(P_v(j))
%   \textcolor{black}{\mathcal{L}_{GRW}  =} & \mathcal{L}_{GRW} + \mathcal{L}_{visit}, 
  \end{aligned}
\label{eq:RW_loss}
\vspace{-2mm}
\end{equation}
% \vspace{-2mm}
where first term minimizes cross entropy loss
between every row in $P^{\mathbf{C } \rightarrow \mathbf{C }}(t,X_u) \forall t=1 \to T$  and uniform distribution over seen classes ${U}_c(j) = {\frac{1}{K^s}, \forall j=1 \cdots K^s}$, where $T$ is a hyperparameter and  $\gamma$ is exponential decay set to $0.7$ in our experiments.  In the  second term, we maximizes the probability of  all the generations  $x^u_i \in X_u$ to be equality visited by the random walk. 
Note that, if we replaced ${U}_c$ by an identity matrix to encourage landing to the starting seen
class, the loss becomes an attraction signal similar to ~\cite{8099557}, which defines its conceptual difference to GRaWD. \emph{We call this version GRaWT, T for aTraction}.  


The second term is called 'visit loss' was proposed in~\cite{8099557} to encourage random walker to visit a large set of unlabeled points.  %We applied it here to our generated deviation examples $X_u$.
We compute the overall probability that each generated point would be visited by any of the seen class  $P_v = \frac{1}{N_u} \sum_{i=0}^{N_c}{P^{\mathbf{C} \rightarrow X_u}_i }$, where $P^{\mathbf{C} \rightarrow X_u}_i$ represents the $i^{th}$ row of the $P^{\mathbf{C} \rightarrow X_u}$ matrix; see Fig.~\ref{fig1approach}. The visit loss is then defined  as the  cross-entropy between $P_v$ and the uniform distribution ${U}_x(j) = {\frac{1}{N^u}, \forall j=1 \cdots N^u}$. Hence, visit loss encourages to visit as many examples as possible from $X_u$ and hence improves learning representation. 




\vspace{0mm}
\subsection{GRaWD Integration with Generative ZSL}  We explicitly explore the unseen/creative space of the generator $G$ with a hallucinated semantic representation $s_u\sim p^u$, where $p^u$ is a probability distribution over unseen classes, aimed to be likely hard negatives to seen classes. To sample $s_u \sim p^u$, we follow the sampling strategy proposed in~\cite{elhoseiny2019creativity} due to its simplicity and effectiveness which picks two seen semantic descriptions at random $s_a, s_b \in \mathcal{S}$. Then we sample  $s^u= \alpha s_a + (1-\alpha) s_b$, 
where $\alpha$ is uniformly sampled between $0.2$ and $0.8$. The values of $\alpha$ near $0$ or $1$ are discarded to avoid sampling semantic descriptions very close to seen classes.  

\noindent \textbf{ Generator $G$ loss. }
% \vspace{-0.5em}
\begin{equation}
\small 
\begin{aligned}
L_G =& {\lambda \mathbb{E}_{X_u \sim \phi(G({s_u}, z))), z \sim p_{z}, s_u \sim {p^u}} [{L}_{GRW}(X_u)]}\\
&- \mathbb{E}_{z \sim {p_{z}, s_u \sim {p^u}}}[D^r(G(s_u, z))]    \\  
&- \mathbb{E}_{z \sim {p_{z}, (s_k,y^s) \sim {p^s}}}[D^r(G(s_k, z))\\
&+ \sum_{k=1}^{K^s} y^s_k log(D^{s,k}(G(s_k, z)))]
%&+  \frac{1}{K^s}\sum_{k=1}^{K^s}|| \mathbb{E}_{z \sim {p_{z}}}[G(s_k, z)] - \mathbb{E}_{x \sim {p^k_{data}}}[x]||^2 
\label{eq:gen}
\end{aligned}
% \vspace{-2mm} 
\end{equation}
where first term is our GRaWD loss. 
The second  and the third terms trick the generator to classify, visual generations from both seen semantic descriptions $s_k$ and unseen semantic descriptions $s_u$, as real.
The fourth term encourages the generator to discriminatively generate visual features conditioned on a given seen class description.  


\noindent \textbf{Discriminator $D$ loss. }
\begin{equation}
\small 
\begin{aligned}
L_D = \hspace{0.1cm}  
 \mathbb{E}_{z \sim {p_{z}, s_u \sim {p^u}}}&[D^r(G(s_u, z)) ] \,\,\,\,\,\,\,\,\,\,\,\\
  + \mathbb{E}_{z \sim {p_{z}}, (s_k,y^s) \sim {p^s}}&[D^r(G(s_k, z))] - \mathbb{E}_{x \sim {p_{d}}}[D^r(x)] \\
+  L_{Lip} -  \frac{1}{2}  \mathbb{E}_{x,y \sim {p_{d}}}&[\sum_{k=1}^{K^s} y_k log(D^{s,k}(x)) ] \\
-  \frac{1}{2} \mathbb{E}_{z\sim p_z, (s_k,y^s) \sim {p^s}}&[\sum_{k=1}^{K^s} y^s_k log(D^{s,k}(G(s_k, z))) ] \\ 
\end{aligned}
\label{eq:disc}
% \vspace{-2mm} 
\end{equation}
where image $x$ and corresponding class one-hot label $y$ are  sampled from the data distribution $p_d$. 
%where $y$ is a one-hot vector encoding of the seen class label for the sampled image $x$
$s_k$ and $y^s$ are
features of a semantic description  
and the corresponding one-hot label sampled from seen classes $p^s$. 
The first three terms approximate Wasserstein distance of the distribution of real features and fake features. The fourth term is the gradient penalty to enforce the Lipschitz constraint: $L_{Lip} =  (||\bigtriangledown_{\tilde{x}} D^r(\tilde{x})||_2 - 1)^2$, where  $\tilde{x}$ is the linear interpolation of the real feature $x$ and the fake feature $\hat{x}$; see~\cite{Gulrajani2017improved}.  The last two terms are classification losses of the  real data and generated features from  semantic descriptions of seen classes.%; see supplementary for more  \emph{{Implementation details}}.

% \noindent \textbf{Test Time.}  We use $G$ to hallucinate generations for unseen classes given their semantic description, where NN-classification can be applied. 
% % \kai{To say sth: different from classifier-based models?}   %conventional classifier could be trained or NN-classification can be applied.    
 
% \kai{\noindent \textup{Evaluation.} Most recent papers will train an extra classifier after training their proposed generative model~\cite{narayan2020latent, han2021contrastive}. This kind of classifier is trained with generated $G$}
\kai{\noindent \textbf{Evaluation.}  Most recent papers will train an extra classifier after training their proposed generative model~\cite{narayan2020latent, han2021contrastive}. In ZSL, this classifier is trained with generated $\tilde{X}_u = G(u_k, z)$ from unseen semantic description $u_k$. While in GZSL, training seen images $X_s$ along with $\tilde{X}_u$ is introduced as input of the extra classifier. We claim accessing unseen information before evaluation is not realistic in pure zero-shot learning. We can not access any prior information before testing. We also find this dataset-specific classifier will hurt the generation ability, and there is no guarantee that a model can learn a good representation of both seen and unseen images. We denote the method with access to unseen information (no matter the labeled semantics or the unlabelled testing images) as semantic transductive ZSL. Following the inductive ZSL settings in~\cite{Elhoseiny_2018_CVPR, elhoseiny2019creativity, elhoseiny2021cizsl++}, we use NN-classification, which avoids accessing any unseen semantic information before the evaluation of unseen images. We denote this setting as \textit{inductive ZSL}.}   

%\noindent \textbf{Training.} 
%\textcolor{blue}{mohamed: makes sense?}
%  We construct two minibatches for training the generator $G$, one from seen classes $s_k$ and one from the hallucinated unseen classes $s_u$ to minimize particular $L_G$ (Eq.~\ref{eq:gen}).  The generator is optimized to fool the discriminator into believing the generated features as real either from hallucinated text $s_u$ or the seen text  $s_k$. In the meantime,  we maximize their entropy over the seen classes if the generated features come from hallucinated text $s_h \sim p^h$ or to the corresponding class if from a real text $s_k$. More implementation details can be found in the supplementary materials.  %During \emph{Test}, the visual features of unseen classes can be synthesized by the generator conditioned on a given unseen text  description $s_u$, as $x_u = G(s_u, z)$. 
%end{equation}We generate 60 generated visual features by sampling different $z$ for the same semantic description $s_u$. We then use the generated features to apply a simple nearest neighbor classifier. 

